HMANet: Hybrid Multi-Axis Aggregation Network for Image Super-Resolution

Transformer-based methods have demonstrated excellent performance on super-resolution visual tasks, surpassing conventional convolutional neural networks. However, existing work typically restricts self-attention computation to non-overlapping windows to save computational costs. This means that Transformer-based networks can only use input information from a limited spatial range. Therefore, a novel Hybrid Multi-Axis Aggregation network (HMA) is proposed in this paper to exploit feature potential information better. HMA is constructed by stacking Residual Hybrid Transformer Blocks(RHTB) and Grid Attention Blocks(GAB). On the one side, RHTB combines channel attention and self-attention to enhance non-local feature fusion and produce more attractive visual results. Conversely, GAB is used in cross-domain information interaction to jointly model similar features and obtain a larger perceptual field. For the super-resolution task in the training phase, a novel pre-training method is designed to enhance the model representation capabilities further and validate the proposed model's effectiveness through many experiments. The experimental results show that HMA outperforms the state-of-the-art methods on the benchmark dataset. We provide code and models at https://github.com/korouuuuu/HMA.

==> sec/Peer-reviewing.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

\section{Peer-reviewing}
\subsection{Reviews}
\label{sec:Reviews}
%
\textbf{~~~~~Reviewer1:}

The paper needs to be improved. The novelty of paper is insufficiency. For example, the main parts of model, such as centered kernel alignment (CKA) and fused attention block (FAB) are proposed by previous works. Besides, the improvement of performance is weakly.

\textbf{Reviewer2:}

\begin{itemize}
\item This manuscript has many typos, e.g., L19: velidate – validate, Figure 2 caption: hight-similarity – high-similarity;
\item Poor English expression;
\item “The HMA comprises hybrid attention blocks (HAB) and grid attention blocks (GAB), aiming to consider both local and global receptive fields.” However, I failed to see any introductions about HAB, which confused me a lot. Also, the idea of GAB has been exploited before (except for the grid shuffle);
\item Lack some insights toward the ill-posed problem. Just combining some structures is not enough for CVPR.
\end{itemize}

\textbf{Reviewer3:}
\begin{itemize}
\item This paper lacks sufficient technical innovation. Currently, there are many manners to improve the performance of image SR by introducing various attention mechanisms into Transformer-based models, such as ESRT (CVPR2022), DAT (ICCV2023), LAA-Transformer (IJCAI2023) etc. More importantly, the pre-training strategy presented in the manuscript has no significant technical contribution and lacks a deeper and more essential analysis;
\item The motivation of this work involves to leveraging the self-similarity of images to enhance the performance of image SR. Although the paper introduces structures e.g., FAB and GAB, for this purpose, it lacks deeper study on self-similarity and adequate validation of these structures to illustrate how image self-similarity is utilized for performance improvement;
\item As for Table 1, the experimental results seem to confirm the conclusion that the performance of the model tends to be better when the pre-training SR scale is close but not equal to the target SR scale. For example:
\textbf{Case 1:} When the pretraining scale is SR$\times$2, the best performance is achieved at SR$\times$3;

\textbf{Case 2:} When the pretraining scale is SR$\times$4, the performance of SR$\times$3 is also relatively good, close to Case 1;

\textbf{Case 3:} When the pretraining scale is SR$\times$3, both SR$\times$2 and SR$\times$4 perform better.

This could indicate the fact that the pretraining for adjacent scales may provide more effective supplementary information, but the authors do not take note of this observation, nor do they delve into the potential reasons.

Additionally, Table 1 does not seem to show the setting of the proposed pretraining strategy, i.e., first pretraining the SR×3 with SR×2 and then pretraining SR$\times$2 and SR$\times$4 with SR$\times$3. Combined with the aforementioned observation, the experiment in this part does not illustrate the effectiveness of the proposed pretraining strategy.
\item Most of the models shown in Table 5 are not pre-trained, the comparison is therefore unfair. To illustrate the effectiveness of the proposed HMA or other structural components, the results of the non-pre-trained version should also be exhibited;
\item The results in Table 2 are not consistent with those in Table 5. The PSNR/SSIM for SR$\times$4 on Urban100 is 27.69/0.8405, but they are 28.69/0.8512 in Table 5. If the difference is caused by the pretraining, then the performance gain in this case is 1.0dB, which significantly exceeds the performance gains from pretraining shown in Table 1;
\item There are some obvious mistakes in the manuscript. For instance, line 133: “In order to further investigate the effect of pretraining on its internal representation, Li et al.” And some spaces are missing. Although tehy are not serious problems, the writing should focus on standardization and rigor.
\end{itemize}

\subsection{Rebuttal}
\label{sec:Rebuttal}
We extend our heartfelt gratitude to the reviewers for their meticulous review and invaluable feedback. In addressing specific queries raised by the reviewers, such as the novelty of the proposed method (highlighted by \textcolor{red}{R1}, \textcolor{green}{R2} and \textcolor{blue}{R3}), identification of writing mistakes in the manuscript (pointed out by \textcolor{green}{R2} and \textcolor{blue}{R3}), and the scrutiny of the methodology analysis (emphasized by \textcolor{blue}{R3}), etc., we provide the following comprehensive responses.

\textbf{Novelty} (@\textcolor{red}{R1}, \textcolor{green}{R2} and \textcolor{blue}{R3}): We appreciate your interest in the novelty of our paper, and we would like to explain your perceived shortcomings in this regard. We propose HMANet, which is dedicated to a more fine-grained multi-scale interaction of the self-similarity features in images. The introduced grid shuffle method encourages the grid attention mechanism to adaptively integrate local similarity information of features, thereby more fully utilizing information from within the image's self-similar features. The channel attention enhances the model's feature representation capability by fusing information from different areas. Previous works overlooked similar information in different local areas of the image, even though they improved model performance by the modified attention mechanisms. Additionally, we present a novel model pre-training strategy that effectively enhances model performance on a limited dataset without altering the model architecture.

\textbf{Typos} (@\textcolor{green}{R2} and \textcolor{blue}{R3}): Thank you for bringing the typos in our manuscript to our attention. In addition, in order to distinguish it from existing papers, we rename Hybrid Attention Blocks (HAB) to Residual Hybrid Transformer Block (RHTB) and describe it in detail. We appreciate your careful review, and we apologize for any oversights in the proofreading process. We will promptly address these issues in the revised manuscript. We will conduct a thorough review of the entire manuscript to identify and rectify any other typos or errors that may be present.

\textbf{Methodology analysis} (@\textcolor{blue}{R3}): We appreciate your attention to the motivations of our work and the suggestion to further investigate the issue of image self-similarity. However, due to constraints imposed by the limitations on article length, we did not delve into this aspect in detail in the main body of the text. In response to your feedback, we intend to incorporate an appendix section in the revised manuscript. The appendix  will thoroughly analyze the role and significance of self-similarity in image super-resolution (SR). we will elaborate on how FAB and GAB effectively leverage the self-similarity of images. This will include discussions on the impact of these structures on image features and how they contribute to performance improvement. We also plan to conduct validation experiments on the pre-training strategy to analyze the impact of different pre-trained models on the current model in the super-resolution task, rather than just using CKA to analyze the feasibility of the method. Additionally, we will supplement the examples and visualizations in appendix.

\textbf{Data inconsistencies} (@\textcolor{blue}{R3}): Thank you for bringing this inconsistency to our attention, and we sincerely apologize for the confusion caused by the inconsistent results in Tables \textcolor{red}{2} and \textcolor{red}{5}. The PSNR and SSIM values reported in Table \textcolor{red}{2} are the results of an untrained strategy. In the revised manuscript, we will modify the results in Table \textcolor{red}{2} to the final results after pre-training for a more intuitive comparison.

\textbf{Comparison of results} (@\textcolor{blue}{R3}): Thank you for your valuable comments on our manuscript. We understand the importance of presenting the non-pre-trained version of HMA in the comparison of results. We will make the following improvements in the revised manuscript: present the results of the non-pre-trained model in Table \textcolor{red}{5} and evaluate the effectiveness of the proposed HMA and other structural components under different strategies. This will give the reader a more comprehensive understanding of the impact of pre-training on model performance. We will discuss in detail the differences between pre-trained and non-pre-trained results in the revised manuscript, which will help clarify the contribution of pre-training.

\textbf{Improvement of performance} (@\textcolor{red}{R1}): Thank you for your feedback on the shortcomings of our manuscript in terms of improved performance. As described by reviewer 2, HMA achieves SOTA in quantitative comparisons, especially on scale factor $\times$3. Compared to the baseline method, HMA was able to improve PSNR by 0.2 to 1.43 dB. We will enhance the comparison with the baseline method in order to illustrate the context of the performance improvement more clearly, including a more detailed discussion of how our method compares to the state-of-the-art and baseline methods. In the revised manuscript, we will also include considerations for future work, discussing potential ways to further improve performance or extend the proposed method to different applications or scenarios.


\textbf{References} (@\textcolor{red}{R1}): Thank you very much for your feedback. We have carefully reviewed and considered the references you provided. We have decided to incorporate the references you suggested to ensure that our argumentation is more comprehensive and robust.

We would like to sincerely thank each reviewer for your comments and insights. These questions and concerns have motivated us to think more fully about this manuscript. We will carefully revise and improve our research work.

\subsection{Change list}
\label{sec:Changes}

\textbf{~~~~(1)}Checking and correcting word spelling and grammar problems.

\textbf{(2)}Fixed HAB and RHTB naming duplication issue

\textbf{(3)}The results in Table1 are modified to the results after using the pre-training strategy, and the results in Table2, Table3, and Table4 are changed to the values without using the pre-training strategy.

\textbf{(4)}Add results without pre-training and add pre-trained model comparisons in Table 4.

\textbf{(5)}Add NTIRE 2024 Image Super-Resolution ($\times$4) Challenge result.












